Revisiting Adversarial Training for ImageNet: Architectures, Training and Generalization across Threat Models

While adversarial training has been extensively studied for ResNet architectures and low resolution datasets like CIFAR, much less is known for ImageNet. Given the recent debate about whether transformers are more robust than convnets, we revisit adversarial training on ImageNet comparing ViTs and ConvNeXts. Extensive experiments show that minor changes in architecture, most notably replacing PatchStem with ConvStem, and training scheme have a significant impact on the achieved robustness. These changes not only increase robustness in the seen $\ell_\infty$-threat model, but even more so improve generalization to unseen $\ell_1/\ell_2$-attacks. Our modified ConvNeXt, ConvNeXt + ConvStem, yields the most robust $\ell_\infty$-models across different ranges of model parameters and FLOPs, while our ViT + ConvStem yields the best generalization to unseen threat models.

==> bigtable.tex <==
\begin{table*}[t]
\centering \small \tabcolsep=.8pt
\extrarowheight=1.5pt
\caption{\textbf{Comparison to SOTA $\ell_\infty$-robust models on ImageNet.} For each model we report the number of parameters, FLOPs, number of epochs of adversarial training (AT), the number of PGD steps in AT, clean and $\ell_\infty, \ell_2, \ell_1$-robust accuracy with $\epsilon_\infty=4/255$, $\epsilon_2=2$, $\epsilon_1=75$ (AutoAttack). Models of similar size are sorted in increasing $\ell_\infty$-robustness. %
Our  \convnext + \cvbk improves by $5.8\%$ %
for small, $7.2\%$
for medium, and $2.8\%$ %
for large models over SOTA.
} \label{tab:scale-up}

\begin{tabular}{L{3.5mm} L{38mm} *{2}{C{10mm}} C{12mm} C{9mm} C{9mm}  |*{2}{C{10mm}} |
*{2}{C{10mm}}
}
& \multirow{2}{*}{Architecture} & Params & FLOPs &\multirow{2}{*}{Source} & \multirow{2}{*}{Ep.} & Adv. &
  
  \multicolumn{4}{c}{Adversarial Tr. wrt $\ell_\infty$
  } \\ %
                  & & (M) & (G)  & & & Steps  & clean & $\ell_{\infty}$ & \textcolor{newgray}{$\ell_{2}$} & \textcolor{newgray}{$\ell_{1}$}
                  \\ %
\toprule
\parbox[t]{3mm}{\multirow{15}{*}{\rotatebox[origin=c]{90}{Small}}} & \resnet-50 & 25.0& 4.1 & \citep{salman2020adversarially} & 100& 3&65.88 &33.18 &\textcolor{newgray}{18.88} &\textcolor{newgray}{3.82}  \\
 & \resnet-50 & 25.0& 4.1& \citep{bai2021are} & 100& 1& 67.44 &35.54 &\textcolor{newgray}{18.16} &\textcolor{newgray}{3.90}  \\
& \vit-S & 22.1& 4.6& \citep{bai2021are} & 100& 1&66.62 &36.56 &\textcolor{newgray}{41.40} &\textcolor{newgray}{21.82}  \\
& \vit-S & 22.1& 4.6 & \citep{debenedetti2022light} & 110& 1& 66.78 &37.88 &\textcolor{newgray}{--} &\textcolor{newgray}{--}  \\
& \vit-S & 22.1& 4.6& \citep{mao2022easyrobust} & 90& 3&65.9 &39.24 &\textcolor{newgray}{32.18} &\textcolor{newgray}{10.54}  \\
& \xcit-S12 & 26.0& 4.8& \citep{debenedetti2022light} & 110& 1&72.34 &41.78 &\textcolor{newgray}{46.20} &\textcolor{newgray}{22.72}  \\
& {\cellcolor{lightgreen}} \vit-S & {\cellcolor{lightgreen}}22.1& {\cellcolor{lightgreen}}4.6 & {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}300 & {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}69.22 & {\cellcolor{lightgreen}}44.04 & {\cellcolor{lightgreen}}\textcolor{newgray}{37.52} & {\cellcolor{lightgreen}}\textcolor{newgray}{15.12}  \\
& RobArch-S & 26.1& 6.3& \citep{peng2023robarch} & 110& 3&70.58 &44.12 &\textcolor{newgray}{39.88} &\textcolor{newgray}{15.46}  \\
& {\cellcolor{lightgreen}} \convnextisoshort-S & {\cellcolor{lightgreen}}22.3& {\cellcolor{lightgreen}}4.3& {\cellcolor{lightgreen}}ours& {\cellcolor{lightgreen}}300& {\cellcolor{lightgreen}}2 &{\cellcolor{lightgreen}}69.04 &{\cellcolor{lightgreen}}44.22 &{\cellcolor{lightgreen}}\textcolor{newgray}{36.64} &{\cellcolor{lightgreen}}\textcolor{newgray}{14.88}  \\
& \convnext-T  & 28.6& 4.5& \citep{debenedetti2022light}& 110& 1&71.60 &44.40 &\textcolor{newgray}{45.32} &\textcolor{newgray}{21.76}  \\
& {\cellcolor{lightgreen}} \convnextisoshort-S + \cvbk & {\cellcolor{lightgreen}}23.0& {\cellcolor{lightgreen}}4.7& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}300& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}70.02 & {\cellcolor{lightgreen}}45.90 & {\cellcolor{lightgreen}}\textcolor{newgray}{49.24} & {\cellcolor{lightgreen}}\textcolor{newgray}{\textbf{27.84}}  \\
& {\cellcolor{lightgreen}}\vit-S + \cvbk & {\cellcolor{lightgreen}}22.8& {\cellcolor{lightgreen}}5.0& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}300&{\cellcolor{lightgreen}} 2& {\cellcolor{lightgreen}}72.56 & {\cellcolor{lightgreen}}48.08 & {\cellcolor{lightgreen}}\textcolor{newgray}{\textbf{50.40}} & {\cellcolor{lightgreen}}\textcolor{newgray}{26.68}  \\
&{\cellcolor{lightgreen}} \convnext-T & {\cellcolor{lightgreen}}28.6& {\cellcolor{lightgreen}}4.5 & {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}300& {\cellcolor{lightgreen}}2&{\cellcolor{lightgreen}}72.40 &{\cellcolor{lightgreen}}48.60 &{\cellcolor{lightgreen}}\textcolor{newgray}{38.02} &{\cellcolor{lightgreen}}\textcolor{newgray}{14.88}  \\
& {\cellcolor{lightgreen}} \convnext-T + \cvbk & {\cellcolor{lightgreen}}28.6& {\cellcolor{lightgreen}}4.6& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}300& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}\textbf{72.72} & {\cellcolor{lightgreen}}49.46 &{\cellcolor{lightgreen}}\textcolor{newgray}{48.42} &{\cellcolor{lightgreen}}\textcolor{newgray}{24.52}  \\ 
& {\cellcolor{lightgreen}} \convnext-T + \cvbk & {\cellcolor{lightgreen}}28.6& {\cellcolor{lightgreen}}4.6& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}300& {\cellcolor{lightgreen}}3& {\cellcolor{lightgreen}}72.70 & {\cellcolor{lightgreen}}\textbf{50.16} &{\cellcolor{lightgreen}}\textcolor{newgray}{49.00} &{\cellcolor{lightgreen}}\textcolor{newgray}{24.16}  \\ \midrule

\parbox[t]{3mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Medium}}} & \wrn-50-2 & 68.9& 11.4& \citep{salman2020adversarially} & 100& 3&68.82 &38.12 &\textcolor{newgray}{22.08} &\textcolor{newgray}{4.48}  \\
 & \resnet-101 & 44.5& 7.9& \citep{mao2022easyrobust}  & 90& 3& 69.52 &41.02 &\textcolor{newgray}{25.62} &\textcolor{newgray}{6.56}  \\
 & \xcit-M12  & 46.0& 8.5& \citep{debenedetti2022light}& 110& 1 &74.04 &45.24 &\textcolor{newgray}{48.18} &\textcolor{newgray}{22.72}  \\
   & {\cellcolor{lightgreen}}\vit-M   & {\cellcolor{lightgreen}}38.8& {\cellcolor{lightgreen}}8.0& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50&{\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}71.72 & {\cellcolor{lightgreen}}47.24 &{\cellcolor{lightgreen}}\textcolor{newgray}{49.02}
  &{\cellcolor{lightgreen}}\textcolor{newgray}{\textbf{29.20}} \\
  & {\cellcolor{lightgreen}}\vit-M + \cvbk  & {\cellcolor{lightgreen}}39.5& {\cellcolor{lightgreen}}8.4& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50&{\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}72.40 & {\cellcolor{lightgreen}}48.80 &{\cellcolor{lightgreen}}\textcolor{newgray}{50.56}
  &{\cellcolor{lightgreen}}\textcolor{newgray}{28.12} \\
   & {\cellcolor{lightgreen}}\convnext-S  & {\cellcolor{lightgreen}}50.1& {\cellcolor{lightgreen}}8.7& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}\textbf{74.10} & {\cellcolor{lightgreen}}52.32 &{\cellcolor{lightgreen}}\textcolor{newgray}{43.84}
  &{\cellcolor{lightgreen}}\textcolor{newgray}{19.52}\\
 & {\cellcolor{lightgreen}}\convnext-S + \cvbk & {\cellcolor{lightgreen}}50.3& {\cellcolor{lightgreen}}8.8& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}\textbf{74.10} & {\cellcolor{lightgreen}}\textbf{52.42} &{\cellcolor{lightgreen}}\textcolor{newgray}{\textbf{50.88}}
  &{\cellcolor{lightgreen}}\textcolor{newgray}{25.64}\\ \midrule
  
\parbox[t]{3mm}{\multirow{14}{*}{\rotatebox[origin=c]{90}{Large}}} & \vit-B & 86.6& 17.6& \citep{mao2022easyrobust} & 90& 3&70.42 &43.02 &\textcolor{newgray}{47.26} &\textcolor{newgray}{27.08}  \\
 & \xcit-L12 & 104.0& 19.0 & \citep{debenedetti2022light}& 110& 1&73.76 &47.60 &\textcolor{newgray}{49.38} &\textcolor{newgray}{23.74}  \\
 & Swin-B  & 87.7& 15.5 & \citep{mao2022easyrobust}& 90& 3&74.76 &48.10 &\textcolor{newgray}{44.42} &\textcolor{newgray}{18.04}  \\
 & RobArch-L & 104.0& 25.7 & \citep{peng2023robarch}& 100& 3&73.46 &48.92 &\textcolor{newgray}{39.48} &\textcolor{newgray}{14.74}  \\
 & {\cellcolor{lightgreen}} \vit-B  & {\cellcolor{lightgreen}}86.6& {\cellcolor{lightgreen}}17.6& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}73.32 & {\cellcolor{lightgreen}}50.02 & {\cellcolor{lightgreen}}\textcolor{newgray}{52.14} & {\cellcolor{lightgreen}}\textcolor{newgray}{\textbf{33.12}}  \\
 & {\cellcolor{lightgreen}} \vit-B + \cvbk & {\cellcolor{lightgreen}}87.1& {\cellcolor{lightgreen}}17.9& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50& {\cellcolor{lightgreen}}2&{\cellcolor{lightgreen}}74.38 &{\cellcolor{lightgreen}}52.58 &{\cellcolor{lightgreen}}\textcolor{newgray}{54.38} &{\cellcolor{lightgreen}}\textcolor{newgray}{31.20}  \\
 & \vit-B  & 86.6& 17.6& \citep{rebuffi2022revisiting} & 300& 2& \textbf{76.62} &53.50 &\textcolor{newgray}{--} &\textcolor{newgray}{--}  \\
 & {\cellcolor{lightgreen}} \convnext-B & {\cellcolor{lightgreen}}88.6& {\cellcolor{lightgreen}}15.4& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}75.62 & {\cellcolor{lightgreen}}54.34 &{\cellcolor{lightgreen}}\textcolor{newgray}{48.52} &{\cellcolor{lightgreen}}\textcolor{newgray}{23.70}  \\
 & {\cellcolor{lightgreen}} \convnext-B + \cvbk & {\cellcolor{lightgreen}}88.8& {\cellcolor{lightgreen}}16.0& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}50&{\cellcolor{lightgreen}} 2& {\cellcolor{lightgreen}}75.32 & {\cellcolor{lightgreen}}54.38 & {\cellcolor{lightgreen}}\textcolor{newgray}{50.06} & {\cellcolor{lightgreen}}\textcolor{newgray}{24.76}
  \\ 
 & {\cellcolor{lightgreen}} \vit-B + \cvbk & {\cellcolor{lightgreen}}87.1& {\cellcolor{lightgreen}}17.9& {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}250& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}76.30 &{\cellcolor{lightgreen}}54.66 &{\cellcolor{lightgreen}}\textcolor{newgray}{\textbf{56.30}} &{\cellcolor{lightgreen}}\textcolor{newgray}{32.06}  \\
  & ConvNeXt-B  & 88.6& 15.4& \citep{liu2023comprehensive}$^*$ 
  & 300& 3& 76.02 &55.82 &\textcolor{newgray}{44.68} &\textcolor{newgray}{21.23} \\
 &   {\cellcolor{lightgreen}} \convnext-B + \cvbk & {\cellcolor{lightgreen}}88.8& {\cellcolor{lightgreen}}16.0 & {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}250& {\cellcolor{lightgreen}}2& {\cellcolor{lightgreen}}75.90& {\cellcolor{lightgreen}}56.14 & {\cellcolor{lightgreen}}\textcolor{newgray}{49.12}
  &{\cellcolor{lightgreen}}\textcolor{newgray}{23.34}   \\ 
  & Swin-B  & 87.7& 15.5&  \citep{liu2023comprehensive}$^*$ 
  & 300& 3& 76.16 &56.16 &\textcolor{newgray}{47.86} &\textcolor{newgray}{23.91} \\
  &   {\cellcolor{lightgreen}} \convnext-B + \cvbk & {\cellcolor{lightgreen}}88.8& {\cellcolor{lightgreen}}16.0 & {\cellcolor{lightgreen}}ours & {\cellcolor{lightgreen}}250& {\cellcolor{lightgreen}}3& {\cellcolor{lightgreen}}75.18& {\cellcolor{lightgreen}}\textbf{56.28} & {\cellcolor{lightgreen}}\textcolor{newgray}{49.40}
  &{\cellcolor{lightgreen}}\textcolor{newgray}{23.60}   \\ 
  \bottomrule
  \multicolumn{5}{l}{$^*$ concurrent work}
\end{tabular} 
\end{table*}

